Multi-scale Dynamics in a Massive Online Social Network

Data confidentiality policies at major social network providers have severely limited researchers' access to large-scale datasets. The biggest impact has been on the study of network dynamics, where researchers have studied citation graphs and content-sharing networks, but few have analyzed detailed dynamics in the massive social networks that dominate the web today. In this paper, we present results of analyzing detailed dynamics in the Renren social network, covering a period of 2 years when the network grew from 1 user to 19 million users and 199 million edges. Rather than validate a single model of network dynamics, we analyze dynamics at different granularities (user-, community- and network- wide) to determine how much, if any, users are influenced by dynamics processes at different scales. We observe in- dependent predictable processes at each level, and find that while the growth of communities has moderate and sustained impact on users, significant events such as network merge events have a strong but short-lived impact that is quickly dominated by the continuous arrival of new users.

==> Makefile <==
# $Id: Makefile,v 1.7 2009/06/20 01:18:01 ale Exp $

LATEX=latex

BIBTEX=bibtex
BIBFILE=zhao.bib social.bib han.bib
PAPER=renren

TEXFILES = \
       renren.tex \
        intro.tex \
	impact.tex \
	network.tex \
	related.tex\
	community.tex\
	preferential.tex\
	netmerge.tex


EPSFIGS = \

EPSGRAPHS = $(wildcard plots/*.eps)

%all:  subdirs $(PAPER).pdf
all: $(PAPER).pdf

subdirs:
	$(MAKE) -C plots

bib:
	$(BIBTEX) pln

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

$(PAPER).pdf: $(PAPER).ps 
	ps2pdf14 $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE) 
	$(LATEX)  renren
	$(BIBTEX) renren
	$(LATEX)  renren
	$(LATEX)  renren

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  renren
	$(BIBTEX) renren
	$(LATEX)  renren

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf

